Autonomy in the Real-World: Autonomous Trajectory Planning for Asteroid Reconnaissance via Stochastic Optimization

This paper presents the development and evaluation of an optimization-based autonomous trajectory planning algorithm for the asteroid reconnaissance phase of a deep-space exploration mission. The reconnaissance phase is a low-altitude flyby to collect detailed information around a potential landing site. Although such autonomous deep-space exploration missions have garnered considerable interest recently, state-of-the-practice in trajectory design involves a time-intensive ground-based open-loop process that forward propagates multiple trajectories with a range of initial conditions and parameters to account for uncertainties in spacecraft knowledge and actuation. In this work, we introduce a stochastic trajectory optimization-based approach to generate trajectories that satisfy both the mission and spacecraft safety constraints during the reconnaissance phase of the Deep-space Autonomous Robotic Explorer (DARE) mission concept, which seeks to travel to and explore a near-Earth object autonomously, with minimal ground intervention. We first use the Multi-Spacecraft Concept and Autonomy Tool (MuSCAT) simulation framework to rigorously validate the underlying modeling assumptions for our trajectory planner and then propose a method to transform this stochastic optimal control problem into a deterministic one tailored for use with an off-the-shelf nonlinear solver. Finally, we demonstrate the efficacy of our proposed algorithmic approach through extensive numerical experiments and show that it outperforms the state-of-the-practice benchmark used for representative missions.

==> herofig.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,341); %set diagram left start at 0, and has height of 341

%Image [id:dp3265958088633012] 
\draw (351.87,266.64) node [rotate=-49.52] %{%\includegraphics[width=77.7pt,height=87.78pt]{figures/asteroid-svgrepo-com}};
{\includesvg[width=77.7pt,height=87.78pt]{figures/asteroid-svgrepo-com}};
%Curve Lines [id:da01808683549900647] 
\draw [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.12 ]   (154.01,229.78) .. controls (167.17,92.22) and (508.17,45.78) .. (570.17,218.5) ;
%Curve Lines [id:da9776484582064175] 
\draw [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (154.01,229.78) .. controls (155.17,112.22) and (496.17,91.5) .. (528.17,220.22) ;
%Shape: Arc [id:dp19559440620010937] 
\draw  [draw opacity=0] (154.15,224.46) .. controls (158.18,166.95) and (244.79,121) .. (351.05,121) .. controls (451.79,121) and (534.87,162.3) .. (546.66,215.59) -- (351.05,228.65) -- cycle ; \draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] (154.15,224.46) .. controls (158.18,166.95) and (244.79,121) .. (351.05,121) .. controls (451.79,121) and (534.87,162.3) .. (546.66,215.59) ;  
%Shape: Arc [id:dp06942973731761493] 
\draw  [draw opacity=0] (346.38,285.4) .. controls (338.62,282.95) and (332.98,275.8) .. (332.92,267.34) .. controls (332.85,256.78) and (341.47,248.15) .. (352.18,248.08) .. controls (362.9,248) and (371.64,256.5) .. (371.72,267.06) .. controls (371.78,275.36) and (366.46,282.46) .. (358.98,285.16) -- (352.32,267.2) -- cycle ; \draw    (346.38,285.4) .. controls (338.62,282.95) and (332.98,275.8) .. (332.92,267.34) .. controls (332.85,256.78) and (341.47,248.15) .. (352.18,248.08) .. controls (362.9,248) and (371.64,256.5) .. (371.72,267.06) .. controls (371.77,274.32) and (367.71,280.66) .. (361.68,283.94) ; \draw [shift={(358.98,285.16)}, rotate = 322.82] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ; 
%Image [id:dp22929860344287034] 
\draw (396.12,120.3) node [rotate=-11.83] 
{\includesvg[width=37.45pt,height=44.5pt]{figures/satellite}};

%Shape: Triangle [id:dp8594862182838614] 
\draw  [draw opacity=0][fill={rgb, 255:red, 110; green, 226; blue, 255 }  ,fill opacity=0.35 ] (290.3,141.18) -- (348,240.91) -- (298.38,250.32) -- cycle ;
%Shape: Triangle [id:dp08463453646789754] 
\draw  [draw opacity=0][fill={rgb, 255:red, 110; green, 226; blue, 255 }  ,fill opacity=0.35 ] (392.76,135.24) -- (392.92,245.21) -- (357.17,243.5) -- cycle ;
%Flowchart: Connector [id:dp19306635519294812] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (367.33,237.14) .. controls (367.33,234.99) and (369.31,233.25) .. (371.75,233.25) .. controls (374.19,233.25) and (376.17,234.99) .. (376.17,237.14) .. controls (376.17,239.28) and (374.19,241.02) .. (371.75,241.02) .. controls (369.31,241.02) and (367.33,239.28) .. (367.33,237.14) -- cycle ;
%Straight Lines [id:da5077329451388208] 
\draw    (325,222) -- (375.75,222.24) ;
\draw [shift={(378.75,222.25)}, rotate = 180.27] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Flowchart: Connector [id:dp3331338045502086] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (318.16,238) .. controls (318.16,235.85) and (320.14,234.11) .. (322.58,234.11) .. controls (325.02,234.11) and (327,235.85) .. (327,238) .. controls (327,240.15) and (325.02,241.89) .. (322.58,241.89) .. controls (320.14,241.89) and (318.16,240.15) .. (318.16,238) -- cycle ;
%Image [id:dp02692852278081692] 
\draw (286.12,124.3) node [rotate=-345.93] 
{\includesvg[width=37.45pt,height=44.5pt]{figures/satellite}};
%\includegraphics[width=37.45pt,height=44.5pt]{satellite.svg}};
%Shape: Rectangle [id:dp20123903460767756] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 110; green, 226; blue, 255 }  ,fill opacity=0.35 ] (21.17,256.5) -- (150.17,256.5) -- (150.17,319) -- (21.17,319) -- cycle ;
%Image [id:dp7087728381495058] 
\draw (130.17,276.25) node  %{\includegraphics[width=22.5pt,height=20.63pt]{gear-svgrepo-com.svg}};
{\includesvg[width=22.5pt,height=20.63pt]{figures/gear-svgrepo-com}};
%Image [id:dp9097971236886926] 
\draw (155.12,220.3) node [rotate=-359.13] {\includesvg[width=37.45pt,height=44.5pt]{figures/satellite}};
%Image [id:dp5591484097497139] 
\draw (213.12,151.3) node [rotate=-58.92] {\includesvg[width=37.45pt,height=44.5pt]{figures/satellite}};
%Image [id:dp3168856160836442] 
\draw (479.12,148.3) node [rotate=-122.81] {\includesvg[width=37.45pt,height=44.5pt]{figures/satellite}};
%Image [id:dp06926474696963214] 
\draw (549.12,215.3) node [rotate=-0.8] {\includesvg[width=37.45pt,height=44.5pt]{figures/satellite}};
%Straight Lines [id:da579130391077314] 
\draw    (22,39) -- (638,37.01) ;
\draw [shift={(641,37)}, rotate = 179.81] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- cycle    ;


% Text Node
\draw (183.61,243.09) node  [font=\Large, opacity=1 ]  {$x_{0}$};
% Text Node
\draw (517.61,242.45) node  [font=\Large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {${\displaystyle x_{f}}$};
% Text Node
\draw (514.61,111.45) node  [font=\Large, color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {${\displaystyle t_{2}}$};
% Text Node
\draw (405.61,79.45) node  [font=\Large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {${\displaystyle t_{2}^{o}}$};
% Text Node
\draw (293.61,79.45) node  [font=\Large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {${\displaystyle t_{1}^{o}}$};
% Text Node
\draw (195.61,107.45) node  [font=\Large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {${\displaystyle t_{1}}$};
% Text Node
\draw (590.96,218.63) node  [font=\Large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {${\displaystyle t_{f}}$};
% Text Node
\draw  [fill={rgb, 255:red, 110; green, 226; blue, 255 }  ,fill opacity=0.36 ]  (359,7) -- (468,7) -- (468,33) -- (359,33) -- cycle  ;
\draw (362,11) node [anchor=north west][inner sep=0.75pt]   [align=left] {{Reconnaissance}};
% Text Node
\draw (36,12) node [anchor=north west][inner sep=0.75pt]   [align=left] {{Approach}};
% Text Node
\draw (111,12) node [anchor=north west][inner sep=0.75pt]   [align=left] {{Preliminary Survey}};
% Text Node
\draw (248,11) node [anchor=north west][inner sep=0.75pt]   [align=left] {{Detailed Survey}};
% Text Node
\draw (479,11) node [anchor=north west][inner sep=0.75pt]   [align=left] {{TAG Rehearsal}};
% Text Node
\draw (591,11) node [anchor=north west][inner sep=0.75pt]   [align=left] {{TAG}};
% Text Node
\draw (111.01,218.43) node  [font=\Large,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {${\displaystyle \mathnormal{t_{0}}}$};
% Text Node
\draw (473,44) node [anchor=north west][inner sep=0.75pt]   [align=left] {{Close Proximity Operations}};
% Text Node
\draw (410,293) node [anchor=north west][inner sep=0.75pt]   [align=left] {{Small Body}};
% Text Node
\draw (26,274) node [anchor=north west][inner sep=0.75pt]   [align=left] {{min }$f( x)$\\{s.t. }$ g(x) \ \leq \ 0$};

\end{tikzpicture}

==> observeconsts.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1, scale = 0.4]
%uncomment if require: \path (0,524); %set diagram left start at 0, and has height of 524

%Straight Lines [id:da3425104175460787] 
\draw [line width=0.75]    (104.29,382.89) -- (530.38,508.8) ;
\draw [shift={(533.26,509.65)}, rotate = 196.46] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (17.86,-8.58) -- (0,0) -- (17.86,8.58) -- cycle    ;
%Straight Lines [id:da7008418204086297] 
\draw    (433.98,56.14) -- (318.77,446.27) ;
\draw [shift={(434.83,53.27)}, rotate = 106.45] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (17.86,-8.58) -- (0,0) -- (17.86,8.58) -- cycle    ;
%Shape: Arc [id:dp7105611940564329] 
\draw  [draw opacity=0] (226.43,314.87) .. controls (244.49,304.05) and (264.93,296) .. (287.13,291.56) .. controls (313.82,286.23) and (340.22,286.68) .. (364.76,292) -- (318.77,446.27) -- cycle ; \draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] (226.43,314.87) .. controls (244.49,304.05) and (264.93,296) .. (287.13,291.56) .. controls (313.82,286.23) and (340.22,286.68) .. (364.76,292) ;
%Straight Lines [id:da08445657187980826] 
\draw    (77,109.3) -- (318.77,446.27) ;
\draw [shift={(77,109.3)}, rotate = 54.34] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 6.7, y radius= 6.7]   ;
%Shape: Arc [id:dp257828102667087] 
\draw  [draw opacity=0] (363.72,292.55) .. controls (383.75,299.63) and (403.09,310.35) .. (420.67,324.75) .. controls (422,325.84) and (423.32,326.94) .. (424.61,328.06) -- (318.77,446.27) -- cycle ; \draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ] (363.72,292.55) .. controls (383.75,299.63) and (403.09,310.35) .. (420.67,324.75) .. controls (422,325.84) and (423.32,326.94) .. (424.61,328.06) ;
%Shape: Arc [id:dp6421582642863644] 
\draw  [draw opacity=0] (175.92,243) .. controls (203.82,226.16) and (235.43,213.65) .. (269.79,206.79) .. controls (352.18,190.32) and (432.76,209.83) .. (492.16,253.75) -- (318.77,446.27) -- cycle ; \draw  [color={rgb, 255:red, 65; green, 117; blue, 5 }  ,draw opacity=1 ] (175.92,243) .. controls (203.82,226.16) and (235.43,213.65) .. (269.79,206.79) .. controls (352.18,190.32) and (432.76,209.83) .. (492.16,253.75) ;
%Shape: Rectangle [id:dp5266548845535792] 
\draw   (327.26,419.15) -- (351.12,426.44) -- (342.63,453.56) -- (318.77,446.27) -- cycle ;
%Straight Lines [id:da24916912498744903] 
\draw    (622.9,107.65) -- (320.78,444.04) ;
\draw [shift={(318.77,446.27)}, rotate = 311.93] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (17.86,-8.58) -- (0,0) -- (17.86,8.58) -- cycle    ;
\draw [shift={(624.9,105.42)}, rotate = 131.93] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (17.86,-8.58) -- (0,0) -- (17.86,8.58) -- cycle    ;
%Straight Lines [id:da707653885801423] 
\draw    (624.9,105.42) -- (318.77,446.27) ;
\draw [shift={(318.77,446.27)}, rotate = 131.93] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 6.7, y radius= 6.7]   ;
\draw [shift={(624.9,105.42)}, rotate = 131.93] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 6.7, y radius= 6.7]   ;

% Text Node
\draw (291,264.38) node  [font=\normalsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-358.71]  {$\textcolor[rgb]{0.82,0.01,0.11}{\theta }\textcolor[rgb]{0.82,0.01,0.11}{_\textrm{si}}$};
% Text Node
\draw (413.58,275.54) node  [font=\normalsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-358.71]  {$\theta _\textrm{emi}$};
% Text Node
\draw (336.4,167.78) node  [font=\normalsize,color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ,rotate=-358.71]  {$\textcolor[rgb]{0.25,0.46,0.02}{\theta }\textcolor[rgb]{0.25,0.46,0.02}{_\textrm{phase}}$};
% Text Node
\draw (36.41,64.59) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {Sun};
% Text Node
\draw (595.86,59.1) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {S/C};
% Text Node
\draw (359.96,14.56) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {Normal Vector};
% Text Node
\draw (475.4,306.91) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {Site Distance\\$\displaystyle =d_\textrm{site}$};
% Text Node
\draw (192.82,464.85) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {Landing Site };


\end{tikzpicture}


==> overviewDARE.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1, scale = 0.6]
%uncomment if require: \path (0,341); %set diagram left start at 0, and has height of 341

%Flowchart: Connector [id:dp12151748537931395] 
\draw  [fill={rgb, 255:red, 227; green, 25; blue, 55 }  ,fill opacity=1 ] (136.59,188.78) .. controls (136.59,186.64) and (138.57,184.9) .. (141.01,184.9) .. controls (143.45,184.9) and (145.43,186.64) .. (145.43,188.78) .. controls (145.43,190.93) and (143.45,192.67) .. (141.01,192.67) .. controls (138.57,192.67) and (136.59,190.93) .. (136.59,188.78) -- cycle ;
%Shape: Arc [id:dp24827211677140582] 
\draw  [draw opacity=0] (141.01,188.78) .. controls (141,188.41) and (141,188.03) .. (141,187.65) .. controls (141,128.2) and (229.22,80) .. (338.05,80) .. controls (446.21,80) and (534.01,127.6) .. (535.09,186.55) -- (338.05,187.65) -- cycle ; \draw  [color= {rgb, 255:red, 227; green, 25; blue, 55 } 
,draw opacity=1 ] (141.01,188.78) .. controls (141,188.41) and (141,188.03) .. (141,187.65) .. controls (141,128.2) and (229.22,80) .. (338.05,80) .. controls (446.21,80) and (534.01,127.6) .. (535.09,186.55) ;  
%Shape: Polygon Curved [id:ds4792180423377095] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.75 ] (271.75,177.25) .. controls (291.75,167.25) and (326.25,152.75) .. (371,183) .. controls (415.75,213.25) and (423.75,251.25) .. (371,243) .. controls (318.25,234.75) and (301,273) .. (281,243) .. controls (261,213) and (251.75,187.25) .. (271.75,177.25) -- cycle ;
%Flowchart: Connector [id:dp06726450595072964] 
\draw  [fill={rgb, 255:red, 227; green, 25; blue, 55 }  ,fill opacity=1 ] (209.59,103.78) .. controls (209.59,101.64) and (211.57,99.9) .. (214.01,99.9) .. controls (216.45,99.9) and (218.43,101.64) .. (218.43,103.78) .. controls (218.43,105.93) and (216.45,107.67) .. (214.01,107.67) .. controls (211.57,107.67) and (209.59,105.93) .. (209.59,103.78) -- cycle ;
%Flowchart: Connector [id:dp39339959805372615] 
\draw  [fill= {rgb, 255:red, 227; green, 25; blue, 55 }  ,fill opacity=1 ] (268.59,86.78) .. controls (268.59,84.64) and (270.57,82.9) .. (273.01,82.9) .. controls (275.45,82.9) and (277.43,84.64) .. (277.43,86.78) .. controls (277.43,88.93) and (275.45,90.67) .. (273.01,90.67) .. controls (270.57,90.67) and (268.59,88.93) .. (268.59,86.78) -- cycle ;
%Flowchart: Connector [id:dp21966087384059685] 
\draw  [fill= {rgb, 255:red, 227; green, 25; blue, 55 }  ,fill opacity=1 ] (379.59,82.78) .. controls (379.59,80.64) and (381.57,78.9) .. (384.01,78.9) .. controls (386.45,78.9) and (388.43,80.64) .. (388.43,82.78) .. controls (388.43,84.93) and (386.45,86.67) .. (384.01,86.67) .. controls (381.57,86.67) and (379.59,84.93) .. (379.59,82.78) -- cycle ;
%Flowchart: Connector [id:dp9349201903619022] 
\draw  [fill= {rgb, 255:red, 227; green, 25; blue, 55 }   ,fill opacity=1 ] (449.59,101.78) .. controls (449.59,99.64) and (451.57,97.9) .. (454.01,97.9) .. controls (456.45,97.9) and (458.43,99.64) .. (458.43,101.78) .. controls (458.43,103.93) and (456.45,105.67) .. (454.01,105.67) .. controls (451.57,105.67) and (449.59,103.93) .. (449.59,101.78) -- cycle ;
%Flowchart: Connector [id:dp6985508942904058] 
\draw  [fill={rgb, 255:red, 227; green, 25; blue, 55 }  ,fill opacity=1 ] (530.67,186.55) .. controls (530.67,184.4) and (532.65,182.66) .. (535.09,182.66) .. controls (537.53,182.66) and (539.51,184.4) .. (539.51,186.55) .. controls (539.51,188.7) and (537.53,190.44) .. (535.09,190.44) .. controls (532.65,190.44) and (530.67,188.7) .. (530.67,186.55) -- cycle ;
%Shape: Arc [id:dp014675215525090324] 
\draw  [draw opacity=0] (323.38,224.4) .. controls (315.62,221.95) and (309.98,214.8) .. (309.92,206.34) .. controls (309.85,195.78) and (318.47,187.15) .. (329.18,187.08) .. controls (339.9,187) and (348.64,195.5) .. (348.72,206.06) .. controls (348.78,214.36) and (343.46,221.46) .. (335.98,224.16) -- (329.32,206.2) -- cycle ; \draw    (323.38,224.4) .. controls (315.62,221.95) and (309.98,214.8) .. (309.92,206.34) .. controls (309.85,195.78) and (318.47,187.15) .. (329.18,187.08) .. controls (339.9,187) and (348.64,195.5) .. (348.72,206.06) .. controls (348.77,213.32) and (344.71,219.66) .. (338.68,222.94) ; \draw [shift={(335.98,224.16)}, rotate = 322.82] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ; 
%Flowchart: Connector [id:dp5883695950169491] 
\draw  [fill= white  ,fill opacity=1 ] (284.75,170.25) .. controls (284.75,168.1) and (286.73,166.36) .. (289.17,166.36) .. controls (291.61,166.36) and (293.59,168.1) .. (293.59,170.25) .. controls (293.59,172.4) and (291.61,174.14) .. (289.17,174.14) .. controls (286.73,174.14) and (284.75,172.4) .. (284.75,170.25) -- cycle ;
%Flowchart: Connector [id:dp5040615288008434] 
\draw  [fill= white,fill opacity=1 ] (354.75,175.25) .. controls (354.75,173.1) and (356.73,171.36) .. (359.17,171.36) .. controls (361.61,171.36) and (363.59,173.1) .. (363.59,175.25) .. controls (363.59,177.4) and (361.61,179.14) .. (359.17,179.14) .. controls (356.73,179.14) and (354.75,177.4) .. (354.75,175.25) -- cycle ;
%Straight Lines [id:da7477464861809366] 
\draw [-{Latex[length=3mm]}]   (296,152) -- (347.75,152.24) ;
%Straight Lines [id:da1262015066197928] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (273.01,86.78) -- (289.17,170.25) ;
%Straight Lines [id:da6100182801250399] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (384.01,82.78) -- (359.17,175.25) ;
%Shape: Rectangle [id:dp699530814266046] 
\draw  [dash pattern={on 4.5pt off 4.5pt}][line width=0.75]  (251,46) -- (410.75,46) -- (410.75,131.25) -- (251,131.25) -- cycle ;
%Straight Lines [id:da2830281734472738] 
\draw[-{Latex[length=5mm]}] (79.75,208.25) -- (80.74,45.25) ;
% Text Node
\draw (122.61,177.09) node  [font=\color{black}, opacity=1 ]  {${\displaystyle x_{t_0}}$};
% Text Node
\draw (419.71,242.23) node [font=\color{black}, anchor=north west][inner sep=0.75pt]  {SB};
% Text Node
\draw (514.61,177.45) node  [font=\color{black},opacity=1 ]  {${\displaystyle x_{t_f}}$};
% Text Node
\draw (464.61,123.45) node  [font=\color{black},,opacity=1 ]  {${\displaystyle t_{2}}$};
% Text Node
\draw (390.61,104.45) node  [font=\color{black},,opacity=1 ]  {${\displaystyle t_{2}^{o}}$};
% Text Node
\draw (278.61,111.45) node  [font=\color{black},,opacity=1 ]  {$t_{1}^{o}$};
% Text Node
\draw (222.61,125.45) node  [font=\color{black}, opacity=1 ]  {${\displaystyle t_{1}}$};
% Text Node
\draw (146.61,210.45) node  [ font=\color{black}, black  ,opacity=1 ]  {${\displaystyle t = 0}$};
% Text Node
\draw (542.61,208.45) node  [font= \normalsize, black ,opacity=1 ]  {${\displaystyle t_{f}}$};
% Text Node

\draw (126.61,62.09) node  [font = \normalsize,opacity=1 ]  {To Sun};

\end{tikzpicture}
